Irregular Repetition Slotted ALOHA in an Information-Theoretic Setting

An information-theoretic approach to irregular repetition slotted ALOHA (IRSA) is proposed. In contrast with previous works, in which IRSA analysis is conducted only based on quantities that are typical of collision models such as the traffic, the new approach also captures more fundamental quantities. Specifically, a suitable codebook construction for the adder channel model is adopted to establish a link with successive interference cancellation over the multi-packet reception channel. This perspective allows proving achievability and converse results for the average sum rate of IRSA multiple access schemes.

==> Figures/converse.tex <==
\tikzset{every picture/.style={line width=0.5pt}} %set default line width to 0.75pt        
\usetikzlibrary{plotmarks}
\pgfplotsset{every axis/.append style={
                    tick label style={font=\small}
                    }}

\newcommand{\oneminuseps}{0.99}
\makeatletter
\tikzset{
    scale plot marks/.is choice,
    scale plot marks/false/.code={
        \def\pgfuseplotmark##1{\pgftransformresetnontranslations\csname pgf@plot@mark@##1\endcsname}
    },
    scale plot marks/true/.style={},
    scale plot marks/.default=true
}
\makeatother

\begin{tikzpicture}
    \begin{axis}[
        xmin=1,
        xmax=6,
        yscale=0.5,
        scale plot marks = false,
        xlabel=$T$,
        ylabel=$R_{\mathrm{sum}}$,
        mark options={solid}]
    
    \addplot[smooth,black,solid,scale plot marks=false] plot coordinates {
        (1,1*\oneminuseps) 
        (10,1*\oneminuseps)}
    ;
    
    %IRSA2
    \addplot[smooth,mark=o,black,densely dashed,scale plot marks=false] plot coordinates {
        (1,0.796812*\oneminuseps) 
        (2,0.930895*\oneminuseps) 
        (3,0.968561*\oneminuseps) 
        (4,0.983682*\oneminuseps) 
        (5,0.990869*\oneminuseps) 
        (6,0.994637*\oneminuseps) 
        (7,0.996742*\oneminuseps) 
        (8,0.997971*\oneminuseps) 
        (9,0.998713*\oneminuseps) 
        (10,0.999171*\oneminuseps)
    };
    %\addlegendentry{Case 1}

    %mixed IRSA2
    \addplot[smooth,color=black,dash dot, mark=o,scale plot marks=false]
        plot coordinates {
            (1,0.830564*\oneminuseps) 
            (2,0.943942*\oneminuseps) 
            (3,0.97469*\oneminuseps) 
            (4,0.986903*\oneminuseps) 
            (5,0.992682*\oneminuseps) 
            (6,0.995705*\oneminuseps) 
            (7,0.997392*\oneminuseps)
            (8,0.998376*\oneminuseps) 
            (9,0.99897*\oneminuseps) 
            (10,0.999337*\oneminuseps)
        };
    %\addlegendentry{Case 2}

    %IRSA3
    \addplot[smooth,color=black,densely dashed,mark=x,scale plot marks=false]
        plot coordinates {
            (1,0.94048*\oneminuseps) 
            (2,0.989525*\oneminuseps) 
            (3,0.997421*\oneminuseps) 
            (4,0.99927*\oneminuseps) 
            (5,0.999777*\oneminuseps) 
            (6,0.999928*\oneminuseps) 
            (7,0.999976*\oneminuseps)
            (8,0.999992*\oneminuseps) 
            (9,0.999997*\oneminuseps) 
            (10,0.999999*\oneminuseps)
        };
    %\addlegendentry{Case 2}
    
    %mixed IRSA3
    \addplot[smooth,color=black,dash dot, mark=x,scale plot marks=false]
        plot coordinates {
            (1,0.95181*\oneminuseps) 
            (2,0.991602*\oneminuseps) 
            (3,0.997936*\oneminuseps) 
            (4,0.999416*\oneminuseps) 
            (5,0.999777*\oneminuseps) 
            (6,0.999943*\oneminuseps) 
            (7,0.999981*\oneminuseps)
            (8,0.999994*\oneminuseps) 
            (9,0.999998*\oneminuseps) 
            (10,0.999999*\oneminuseps)
        };
    %\addlegendentry{Case 2}
    
    \end{axis}

\end{tikzpicture}
